Intervention-Robust VLA: Diverse Demonstrations for Robot Deployment with Safety Filters

Vision-Language-Action models (VLAs) have shown strong potential for learning complex robotic behaviors from demonstrations. However, learning safe behavior directly from data requires extensive coverage of safety-critical situations, which is often impractical in real-world settings. Test-time safety filters provide an alternative by correcting unsafe actions during deployment, but these interventions can drive the robot into states poorly covered by the training data, thereby degrading task performance. We introduce InteR-VLA, an intervention-robust framework for VLAs that leverages diverse task-completing demonstrations to broaden task-relevant state coverage and maintain competence under safety interventions. By better aligning the training distribution with safety-filtered deployment under the same data budget, our approach mitigates intervention-induced distribution shift while preserving task performance. Real-world experiments across in-distribution and out-of-distribution settings show that InteR-VLA maintains safety, increases Safe Success Rate up to 90% from 0% for nominal policies, and consistently outperforms nominal-data training on both evaluated VLAs.

==> preamble_snippet.tex <==
% ============ InteR-VLA figure style (paste into main.tex, right after the ============
% ============ "Define Colors Palette" \definecolor block)                   ============
% One place for every plot's look: font, chrome colours, strategy styles. Figures 4, 6, 7
% use it. Font: IBM Plex Mono Regular (+ the Plex Sans pi), bundled in fonts/ (OFL 1.1) so
% the build does not depend on the TeX installation having the `plex` package (Overleaf's
% build fell back to Computer Modern). Private family names, so \ttfamily, \url and the body text
% are untouched.
\usepackage[LGR,OT1]{fontenc}  % LGR only for the upright Plex pi in figures; OT1 (listed
                               % last) stays the document encoding, exactly as before
\definecolor{fig_edge}{HTML}{2B2B2B}   % bar edges, marker edges
\definecolor{fig_grid}{HTML}{E3E6EA}   % horizontal grid
\definecolor{fig_rule}{HTML}{C9CFD6}   % dashed group separators
\definecolor{fig_ink}{HTML}{1A1A1A}    % all text
\definecolor{fig_muted}{HTML}{6E6E6E}  % the "0" of a measured zero, notes
% Strategy -> colour. Colour encodes the data-collection strategy ONLY.
\colorlet{strat_vla_normal}{purple_light}   % VLA (Normal)
\colorlet{strat_sf_normal}{green_light}     % VLA-SF (Normal)
\colorlet{strat_sf_diverse}{blue_med}       % VLA-SF (Diverse)
\colorlet{strat_sf_multi}{org_med}          % VLA-SF (Multi) - the accent, drawn last
% \figfont{<pt>}: the one figure face at a printed size (figures are never scaled)
\DeclareFontFamily{OT1}{irvlaMono}{\hyphenchar\font=-1}
\DeclareFontShape{OT1}{irvlaMono}{m}{n}{<-> fonts/irvla-mono}{}
\DeclareFontFamily{LGR}{irvlaPi}{}
\DeclareFontShape{LGR}{irvlaPi}{m}{n}{<-> fonts/irvla-pi}{}
\pdfmapline{=irvla-mono plxMono " AutoEnc_lxmhqhn4noowsq3ysicmnkmtrh ReEncodeFont " <[fonts/irvla-mono.enc <fonts/irvla-mono.pfb}
\pdfmapline{=irvla-pi plxSans " AutoEnc_5wdxh7ymgkufbhnkeefuvaxvnh ReEncodeFont " <[fonts/irvla-pi.enc <fonts/irvla-pi.pfb}
\newcommand{\figfont}[1]{\fontencoding{OT1}\fontfamily{irvlaMono}\fontseries{m}%
  \fontshape{n}\fontsize{#1}{#1}\selectfont}
\newcommand{\figpi}{{\fontencoding{LGR}\fontfamily{irvlaPi}\fontseries{m}%
  \fontshape{n}\selectfont p}}            % Plex Mono has no Greek; Plex Sans' pi
\newcommand{\figpizero}{\figpi\raisebox{-0.35ex}{\figfont{5.3}0.5}}
\pgfplotsset{
  % shared chrome: 0-1 rate axis, ticks 0/.5/1, light grid, open top and right
  irvla/.style={
    scale only axis, clip=false,
    axis x line*=bottom, axis y line*=left,
    axis line style={line width=0.6pt, draw=fig_ink!85},
    ymin=0, ymax=1, ytick={0,0.5,1},
    ymajorgrids, grid style={fig_grid, line width=0.5pt},
    tick align=outside, major tick length=2.5pt, tick style={line width=0.6pt, fig_ink!85},
    ticklabel style={font=\figfont{7.5}, text=fig_ink},
    % numeric ticks in the figure face (not the math font); y ticks read 0 / .5 / 1
    xticklabel={\pgfmathprintnumber[assume math mode=true]{\tick}},
    yticklabel={\pgfmathprintnumber[assume math mode=true, skip 0.]{\tick}},
    label style={font=\figfont{8.5}, text=fig_ink},
    title style={font=\figfont{8.5}, text=fig_ink},
    legend style={draw=none, fill=none, font=\figfont{7.5}, text=fig_ink},
  },
  irvla bar/.style={draw=fig_edge, line width=0.7pt, fill=#1},
  irvla line/.style={color=#1, line width=1.3pt, mark=*, mark size=2.1pt,
    mark options={solid, fill=#1, draw=fig_edge, line width=0.56pt}},
  % value label: 1.2pt above the bar top, no leading zero (.80), a zero prints a grey 0
  irvla value/.style={
    nodes near coords={\pgfmathfloatifflags{\pgfplotspointmeta}{0}%
      {\textcolor{fig_muted}{0}}%
      {\pgfmathprintnumber[fixed, fixed zerofill, precision=2, skip 0.,
                           assume math mode=true]{\pgfplotspointmeta}}},
    every node near coord/.append style={font=\figfont{6.5}, text=fig_ink,
      anchor=base, yshift=1.2pt, inner sep=0pt},
  },
}
% ===================================================================================

